Differentially Private Learning Needs Hidden State (Or Much Faster Convergence)

Prior work on differential privacy analysis of randomized SGD algorithms relies on composition theorems, where the implicit (unrealistic) assumption is that the internal state of the iterative algorithm is revealed to the adversary. As a result, the R\'enyi DP bounds derived by such composition-based analyses linearly grow with the number of training epochs. When the internal state of the algorithm is hidden, we prove a converging privacy bound for noisy stochastic gradient descent (on strongly convex smooth loss functions). We show how to take advantage of privacy amplification by sub-sampling and randomized post-processing, and prove the dynamics of privacy bound for "shuffle and partition" and "sample without replacement" stochastic mini-batch gradient descent schemes. We prove that, in these settings, our privacy bound converges exponentially fast and is substantially smaller than the composition bounds, notably after a few number of training epochs. Thus, unless the DP algorithm converges fast, our privacy analysis shows that hidden state analysis can significantly amplify differential privacy.

==> appendices/append_pseudocode_mBGD.tex <==
\begin{algorithm}[ht]
	\caption{$\algo_{\text{Noisy-mBGD}}$: Noisy mini-batch Gradient Descent}
	\label{alg:noisymBGD}
	\begin{algorithmic}
		\STATE {\bfseries Input:} Data domain $\X$. Dataset $\D = (\x_1, \x_2, \cdots, \x_\size)$ with $\x_i\in\Domain$. A convex parameter set $\C\subseteq\mathbb{R}^\dimension$ in Euclidean space. A loss function $\loss(\vtheta;\x)$ over $\C\times\X$ with gradient sensitivity $\lVert\nabla\ell(\theta,\x) - \nabla\ell(\theta,\x')\rVert_2\leq S_g$, learning rate schedule $\step_\kk^{j}$ and noise standard deviation schedule $\sig_\kk^{j}$ for $\kk=0, \cdots,\K-1$ and $j = 0, \cdots, n/b - 1$, parameter initialization $\vtheta_0$, mini-batch size $b$.
		\STATE{\bfseries Initialization:} $\theta_{0}^{0} = \theta_0$
		\FOR {$\kk = 0, 1, \cdots, \K - 1$}
		\STATE{\bfseries Batch generation:} form $n/b$ non-overlapping mini-batch subsets of $[n]$ with size $b$: $B_\kk^0, \cdots, B^{n/b-1}_\kk$.\label{step:batch_generation}
		\FOR {$j = 0, 1, \cdots, n/b - 1$}
		\STATE {$\g{\vtheta_{\kk}^{ j}}{\B^{j}_\kk}= \frac{1}{b}\sum_{x_\ii\in \B_\kk^{j}} \grad\loss(\vtheta_{\kk}^{j};\x_\ii)$}
		\STATE {$\vtheta_{\kk}^{j + 1} = \vtheta_{\kk}^{j} - \step_{\kk}^j\cdot \g{\vtheta_{\kk}^{j}}{\B_{\kk}^j} + \sqrt{2\step_\kk^j}\cdot \noise_{\kk}^j\cdot \Gauss{0}{\Id}$} \label{alg:ngd:updatestep}
		\ENDFOR
		\STATE {$\vtheta_{\kk + 1}^{0} = \vtheta_{\kk}^{n/b}$}
		\ENDFOR
		\STATE {Output $\vtheta_{\K}^{0}$}
	\end{algorithmic}
\end{algorithm}

==> packages_and_commands.tex <==
%\usepackage{times}
\usepackage[numbers]{natbib}
\usepackage{authblk}        % authors
\usepackage[T1]{fontenc} \usepackage{ae} \usepackage{aecompl}
\usepackage[utf8]{inputenc}
\usepackage{hyperref}
\usepackage{url}

\usepackage{amsmath,amssymb,amsthm}
\usepackage{mathtools}
\usepackage[margin=1.1in]{geometry} % for page margin
\usepackage{algorithm}  % for algorithms
% \usepackage{algorithmic}
\usepackage[noend]{algpseudocode}  % for algorithms

\usepackage[capitalize,noabbrev]{cleveref}
\crefformat{footnote}{#2\footnotemark[#1]#3}

\usepackage{subcaption}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALGORITHMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{multirow}
\usepackage{booktabs}

\usepackage{tablefootnote}

\usepackage{caption}
\captionsetup{font=small}

\PassOptionsToPackage{linktocpage}{hyperref}

\usepackage[hyperindex,breaklinks]{hyperref}

==> sections/sec_prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

\subsection{Differential Privacy} 

Differential privacy originates from~\citet{dwork2006calibrating}.  However, many follow-up variants of differential privacy, such as R\'enyi differential privacy~\cite{mironov2017renyi}, concentrated differential privacy~\cite{dwork2016concentrated, bun2016concentrated} and Gaussian differential privacy~\cite{dong2019gaussian}, are also actively used to quantify and bound the privacy loss of algorithms. In this paper, we focus on proving standard $(\eps,\delta)$-differential privacy guarantee, and also the R\'enyi differential privacy guarantee, for differentially private learning. 

\begin{definition}[Neighboring Datasets]
	Let $D$ and $D'$ be two datasets with the same size that consist of $n$ records. We say $D$ and $D'$ are neighboring datasets if they differ in at most one data record.
\end{definition}

%We acknowledge that there is also another definition of neighboring datasets where $D$ and $D'$ are not of the same size.

\begin{definition}[Differential Privacy~\cite{dwork2006calibrating, dwork2014algorithmic}]
    A randomized algorithm $\mathcal{A}$ is $(\eps,\delta)$-differentially private (or $(\eps,\delta)$-DP for short), if for any neighboring datasets $D$ and $D'$, and for all possible event $S$ in the output space of $\mathcal{A}$, it holds that
    %
    \begin{align}
        P\left(\mathcal{A}(D)\in S\right) \leq e^\eps\cdot P\left(\mathcal{A}(D')\in S\right) + \delta
    \end{align}
\end{definition}

\begin{definition}[R\'enyi divergence]
    \label{def:Renyidivergence}
    For two distributions $\mu$ and $\nu$ with density $\mu(\theta)$ and $\nu(\theta)$ on $\theta\in\mathbb{R}^d$, the R\'enyi divergence of order $\alpha>1$ of $\mu$ with respect to $\nu$ is
    %
    \begin{align}
        R_\alpha(\mu\lVert \nu) = \frac{1}{\alpha -1}\log \mathbb{E}_{\theta\sim\nu}\left[\left(\frac{\mu(\theta)}{\nu(\theta)}\right)^\alpha\right]
    \end{align}
\end{definition}

\begin{definition}[$(\alpha,\eps)$-R\'enyi DP~\cite{mironov2017renyi}]
    A randomized algorithm $\mathcal{A}$ is said to satisfy $(\alpha, \eps)$-R\'enyi differential privacy (or $(\alpha,\eps)$-R\'enyi DP for short), if for any neighboring datasets $D$ and $D'$, it holds that
    %
    \begin{align}
        R_\alpha(\mathcal{A}(D)\lVert \mathcal{A}(D')) \leq \eps,
    \end{align} 
	%
    where $\mathcal{A}(D)$ and $\mathcal{A}(D')$ denote the distribution of outputs given input dataset $D$, and $D'$ respectively, and $R_{\alpha}(\mu\lVert \nu)$ is the R\'enyi divergence defined in \cref{def:Renyidivergence}.
\end{definition}

\subsection{Log-Sobolev Inequality} 

The logarithmic Sobolev inequalities for distributions have various origins in mathematical physics~\cite{gross1975logarithmic}, quantum field theory~\cite{federbush1969partially}, and information theory~\cite{stam1959some}. In this paper, we follow \citet{vempala2019rapid} and use the following definition for log-Sobolev inequality with constant $c$.

\begin{definition}[log-Sobolev inequality with constant $c$]
    A distribution $\nu$ with density $\nu(\theta)$ over $\theta\in\mathbb{R}^d$ satisfies the log-Sobolev inequality (LSI) with constant $c$ if for all smooth function $g:\mathbb{R}^d\rightarrow \mathbb{R}$ with $\mathbb{E}_{\theta\sim\nu}\left[g(\theta)^2\right]<\infty$,
    \begin{align}
        \mathbb{E}_{\theta\sim\nu}\left[g(\theta)^2\log\left( g(\theta)^2\right)\right] - \mathbb{E}_{\theta\sim\nu}\left[g(\theta)^2\right]\cdot \log \mathbb{E}_{\theta\sim\nu}\left[g(\theta)^2\right]\leq \frac{2}{c}\mathbb{E}_{\theta\sim\nu}\left[\lVert \nabla g(\theta)\rVert^2\right].
    \end{align}
\end{definition}
